Few-shot Action Recognition with Permutation-invariant Attention

Many few-shot learning models focus on recognising images. In contrast, we tackle a challenging task of few-shot action recognition from videos. We build on a C3D encoder for spatio-temporal video blocks to capture short-range action patterns. Such encoded blocks are aggregated by permutation-invariant pooling to make our approach robust to varying action lengths and long-range temporal dependencies whose patterns are unlikely to repeat even in clips of the same class. Subsequently, the pooled representations are combined into simple relation descriptors which encode so-called query and support clips. Finally, relation descriptors are fed to the comparator with the goal of similarity learning between query and support clips. Importantly, to re-weight block contributions during pooling, we exploit spatial and temporal attention modules and self-supervision. In naturalistic clips (of the same class) there exists a temporal distribution shift--the locations of discriminative temporal action hotspots vary. Thus, we permute blocks of a clip and align the resulting attention regions with similarly permuted attention regions of non-permuted clip to train the attention mechanism invariant to block (and thus long-term hotspot) permutations. Our method outperforms the state of the art on the HMDB51, UCF101, miniMIT datasets.

==> 3831 2/0-abstract.tex <==
\begin{abstract}
Many few-shot learning models focus on recognising images.  
In contrast, we tackle a challenging task of few-shot action recognition from videos.  We build on a C3D encoder for spatio-temporal video blocks to capture short-range action patterns. Such encoded blocks are aggregated by permutation-invariant pooling to make our approach robust to varying action lengths and long-range temporal dependencies whose patterns are unlikely to repeat even in clips of the same class. Subsequently, the pooled representations are combined into simple relation descriptors which encode so-called query and support clips. Finally, relation descriptors are fed to the comparator with the goal of similarity learning between query and support clips. Importantly, to re-weight block contributions during pooling, we exploit spatial and temporal attention modules and self-supervision. In naturalistic clips (of the same class) there exist a temporal distribution shift--the locations of discriminative temporal action hotspots vary. Thus, we permute blocks of a clip and align the resulting attention regions with similarly permuted attention regions of non-permuted clip to train the attention mechanism invariant to block (and thus long-term hotspot) permutations. Our method outperforms the state of the art on the HMDB51, UCF101,  \textit{mini}MIT datasets.
\end{abstract}

==> 3831 2/1-introduction.tex <==
\section{Introduction}

Few-shot learning is an open problem with the goal to design algorithms that learn in the low-sample regime. Examples include meta-learning  \cite{finn2017model,lee2019meta,antoniou2018train,Simon_2019_NIPS,Simon_2020_CVPR},  robust feature representations by relation learning \cite{snell2017prototypical,sung2017learning,wertheimer2019few,zhang2019power}, gradient-based \cite{Zintgraf2019Cavia,Rusu2019LEO,Simon_2020_ECCV} and  hallucination strategies for insufficient data \cite{hariharan2017low,zhang2019few}. %The ultimate goal of few-shot learning is to design neural networks which could be trained effectively without large scale datasets.  

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fsar_demo}
    \caption{Augmentation-guided attention by alignment. Fig. \ref{fig:demo}a shows that discriminative action blocks (in red, top left) may be misaligned with discriminative action blocks of test clip (in blue, bottom left). If the attention unit observes different distributions of locations of discriminative blocks at training and testing time, it fails. With the right approach, one may overcome the distribution shift (top and bottom right panels). Fig. \ref{fig:demo}b shows how the augmentation-guided attention by alignment works for permutation-based augmentations: (i) we shuffle training  blocks of a clip to train an attention on permuted blocks, (ii) we shuffle in the same way coefficients of the attention vector from the non-permuted blocks. Both attention vectors are then encouraged to align by a dedicated loss term during training. Fig. \ref{fig:demo}c shows histograms of alignment-errors on test data. The top histogram shows larger errors (no alignment loss used in training) while the bottom histogram shows small errors (alignment during testing improves).
    }
    \label{fig:demo}
\end{figure}

%While the majority of existing few-shot learning approaches focus on the image-level recognition, 
However, very few papers address video-based few-shot learning.  As annotating large video datasets is prohibitive, this makes the problem we study particularly valuable.  While results are far from satisfactory on {\em Kinetics} \cite{i3d_net}, the largest action recognition dataset, its size of 300,000 video clips with hundreds of frames each exceeds the size of large-scale image %classification datasets such as 
ImageNet \cite{ILSVRC15} and Places205 \cite{places_dataset} datasets. %Yet, the state of the art in action recognition is far from satisfactory \cite{i3d_net}.

There exist few limited works on few-shot learning for action recognition \cite{mishra2018generative,xu2018dense,guo2018neural,Zhu_2018_ECCV}. However, they focus on modeling 3D body joints with graphs \cite{guo2018neural}, attribute-based learning in generative models \cite{mishra2018generative},   network design for low-sample classification \cite{xu2018dense} and salient memory approach \cite{Zhu_2018_ECCV}. In contrast, we focus on robust  relation/similarity, spatial and temporal modeling of short- and long-term range action patterns via permutation-invariant pooling and attention. % Most of them focus on the aspect of network design, but without in-depth analysis of various aspects of the specific video domain. 

To obtain a robust few-shot action recognition approach, we investigate how to: (i) represent discriminative short- and non-repetitive long-term action patterns for relation/similarity learning, (ii) localize temporally  discriminative action blocks with limited number of training samples, and (iii) deal with long-term temporal distribution shift of such discriminative patterns (these patterns never re-appear at the same temporal locations even for clips of the same class).

\footnotetext{\label{foot:selfsup}Self-supervision assumes generating cheap-to-obtain data (\eg, augmentation by rotations) from the original data and imposing an auxiliary task whose goal is to predict the label of  an augmentation with the goal of robust representation learning \cite{dosovitskiy2014discriminative,doersch2015unsupervised,gidaris2018unsupervised,jian2019evolutionarily,jian2020representation}. We are first to apply the self-supervision by alignment paradigm to the problem of robust attention training (we devise an augmentation-guided attention).}

To address the first point, our early experiments indicated that short-term discriminative action patterns can be captured by an encoder with  C3D convolutional blocks. Thus, resulting features from a clip undergo permutation-invariant pooling which discards long-term non-repetitive dependencies. Finally, pooled query/support representations form relation descriptors are fed into a comparator.

Regarding the second point, aggregating  spatio-temporal blocks with equal weights is suboptimal. Thus, we devise spatial/temporal attention units to emphasize discriminative blocks. Under the low-sample regime, self-supervision by {\em jigsaw} and {\em rotation} \footnotemark[\getrefnumber{foot:selfsup}] helps train a more robust  encoder, comparator and attention. However, vanilla attention (and/or  self-supervision) cannot fully promote the invariance to temporal (or spatial) permutations as described next.

To address the third point, we note that long-term dependencies in clips are non-repetitive \eg, videos of the same class often contain relevant action blocks at different temporal locations. Figure \ref{fig:demo}a shows that discriminative blocks of training and testing clips of {\em dance} class do not align (top left \vs bottom left corner). By permuting the blocks of training (top right), one can make them align with the most discriminative test samples (bottom right). Figure \ref{fig:demo}b shows that for a given clip, we (i) shuffle its blocks and feed them to the attention mechanism (shuffling pass), (ii) we shuffle accordingly the attention coefficients from a non-shuffled pass through attention, and (iii) we force attention coefficients from both passes to align. Such an attention by alignment deals with the distribution shift of discriminative temporal (and spatial) patterns via {\em jigsaw} augmentation (but applies also to {\em rotation, zoom}, \etc) 
%
% This mechanism can be considered a form of self-supervision, where various augmentations are introduced with the goal of attention identifying regions of interest in both augmented and the original clips, while the auxiliary loss is tasked with unrolling these augmentations such that the discrepancy between the attention maps is minimized. 
%
%To answer the above questions, we propose an improved self-supervised attention mechanism for few-shot action recognition, which simultaneously uses attention modules to localize the actions to improve the accuracy, and feeds numbers of augmented clips into the network with self-supervised loss to enrich training data patterns and improve  robustness of model. Figure \ref{fig:demo} illustrates our idea. Firstly, we impose spatial and temporal attention mechanisms in feature space to detect the frames of interest and regions of interest for action relation learning, thus highlighting the key information and discarding noisy/uninformative background information. Secondly, we apply extensively augmentations on action clips and train a self-supervised discriminator to recognize the augmentation patterns. By providing plentiful patterns of action videos to the network, we can effectively improve the robustness of our few-shot model and reduce its uncertainty.
%
%In this paper, we take a deeper look at the few-shot action recognition from the two above-mentioned aspects, propose to simultaneously impose temporal and spatial attention modules to detect the regions and frames of interests, properly refine action representations. Additionally, we employ an extra discriminator to predict the augmentation patterns of given data, \eg, rotation degrees, jigsaw patterns and shuffling orders in self-supervised manner, thus boosting the quality of features extracted from feature encoder. Following we apply second-order pooling on the convolutional features to effectively aggregate them over both temporal and spatial modes. In this way, we extract the co-occurrence matrix given refined features neglecting the temporal orders and spatial positions, which is proved to be much more beneficial for action relation learning.
%
%Furthermore, we apply self-supervision to encourage the attention maps to be robust and consistent in the sense that a robust attention mechanism should  be invariant to both  temporal and spatial augmentations  so that the important spatial/temporal regions matching between augmented and original video pairs could be consistently identified by the attention mechanism irrespective of their actual spatial/temporal locations. However, using a vanilla attention mechanisms without any designated loss cannot guarantee this important property. 
%
 %thus contributing to the augmentation-invariant attentions without extra costs on labeling or training.
%
%Different with previous attention-related works, we are the first proposing to boost the temporal and spatial attentions with self-supervision. It is known that attention is leveraged to detect the key spatial points or temporal frames, however, these keypoints are not robust to data variations, \eg, rotation, jigsaw, as these augmentations are not taken into account in previous works. Applying self-supervision to align attention maps, theoretically we can obtain augmentation-invariant attention maps, which has stronger robustness and lower uncertainty to against the domain-shift and the small number of training sample. Therefore boosting attention with self-supervision is a meaningful and interesting attempt in case current attention-related works use it but know nothing about it. Self-supervised attention enhancement is proved to be more robust and informative than the classic unconscious attention in our evaluations. Last but not least, we propose the unified evaluation protocols on three popular action recognition datasets, which contributes to easier fair comparisons with other future works.
%
To summarize, our contributions include:
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item  A robust pipeline with a C3D-based encoder capturing short-term dependencies which yields block representations subsequently aggregated by permutation-invariant pooling into fixed-length representations which form relation descriptors for relational/similarity learning in an episodic setting \cite{sung2017learning}.
    %
    \item Spatial and temporal attention units which re-weight block contributions during the aggregation step. To improve training of the encoder, comparator and the attention unit  under the low-sample regime, we introduce spatial and temporal self-supervision by {\em rotations}, and {\em spatial} and {\em temporal jigsaws}.
    %
    \item  An improved self-supervised attention unit by applying augmentation patterns such as {\em jigsaws} and/or {\em rotations} on the input of the attention unit and aligning the output with augmented the same way attention vector coefficients from non-augmented data passed by the attention unit\footnotemark[\getrefnumber{foot:selfsup}]. Thus, the attention unit becomes invariant to a given augmentation action by design.
    %
    \item We propose new data splits for a systematic comparison of few-shot action recognition algorithms and we make them available as existing approaches use each different pipeline concepts, data modality, data splits and  protocols\footnote{Section \ref{sec:contrast} explains that existing works do not specify class/validation splits which yields $\sim$6\% variations in accuracy rendering their protocols highly inaccurate. Section \ref{sec:issue} explains this issue  and how we compare our method to existing works.}.
\end{enumerate}

% To the best of our knowledge, this is the first work which incorporates self-supervision into few-shot action recognition, and also the first attempt to use self-supervised attention to produce augmentation-invariant attention maps. 
% Extensive experiments demonstrate the effectiveness of our proposed approach for few-shot action recognition.

==> 3831 2/2-relatedwork.tex <==
\section{Related work}
\label{sec:related}

Below, we discuss zero-, one- and few-shot learning models followed by a discussion on self-supervised learning and second-order pooling.

% \subsection{Learning From Few Samples}
% \label{sec:related_few_shot}

%For deep learning algorithms, the ability of {\em``learning quickly from only a few examples is definitely the desired characteristic to emulate in any brain-like system''} \cite{book_nip}. This desired operating principle poses a challenge to typical CNN-based big data approaches \cite{ILSVRC15} designed for large scale visual category learning. Current trends in computer vision highlight the need for {\em ``an ability of a system to recognize and apply knowledge and skills learned in previous tasks to novel tasks or new domains, which share some commonality''}. 
%This problem was introduced in 1901 under a notion of ``{\em transfer of particle}''~\cite{woodworth_particle} and is closely related to zero-shot learning \cite{larochelle2008zero,farhadi2009describing,akata2013label} which can be defined as an ability to generalize to unseen class categories from categories seen during training. For one- and few-shot learning, some ``{\em transfer of particle}'' is also a desired mechanism as generalizing from one or few datapoints to account for intra-class variability of thousands images is a formidable task.

\noindent{\textbf{One- and few-shot learning}} models have been widely studied in both the shallow \cite{miller_one_example,Li9596,NIPS2004_2576,BartU05,fei2006one} and  deep learning pipelines \cite{koch2015siamese,vinyals2016matching,snell2017prototypical,finn2017model,snell2017prototypical,sung2017learning}. 
Motivated by the human ability to learn new concepts from few samples, early works \cite{fei2006one,lake_oneshot} employ generative models with an iterative inference. %in order to take advantage of knowledge from previously learned tasks. 
%
Siamese Network \cite{koch2015siamese} is a two-stream convolutional neural network  which generates image descriptors and learns the similarity between them. 
%
Matching Network \cite{vinyals2016matching}  proposes query-support episodic learning and $L$-way $Z$-shot learning protocols\footnote{Kindly see \cite{vinyals2016matching,snell2017prototypical,sung2017learning} for the concept of query, support and episodic learning, and the evaluation protocols which  differ from traditional recognition and low-shot learning.}. The similarity between a query and support images is learnt for each episode. At the testing time, each test query (of novel class) is compared against a handful of annotated test support images for rapid recognition. %Thus, images representing novel class concepts unseen during training can be classified with ease. 
%
%It learns to simulate the relations between testing and support images, thus casting the one-shot learning problem as set-to-set learning.
%
Prototypical Networks \cite{snell2017prototypical}  compute distances between a datapoint and class-wise prototypes. %
%
Model-Agnostic Meta-Learning (MAML) \cite{finn2017model} %introduces a meta-learning model which %can be considered a form of transfer learning. %as otherwise fine-tuning on few datapoints per classes is challenging.
%Their model 
is trained on multiple  learning tasks. %This results in a good initial condition for the solver to generalize to other novel tasks. % with few training samples. 
%
Relation Net \cite{sung2017learning} %proposes a simple but
learns relations between query and support images, %. This model is similar to Matching Network \cite{vinyals2016matching} but 
and it leverages a similarity learning neural network to compare query-support pairs. 
%
SalNet \cite{zhang2019few} uses saliency-guided end-to-end sample hallucination to grow the training set. 
%
Graph Neural Networks (GNN) have also been used in few-shot learning \cite{gnn,Kim_2019_CVPR,Gidaris_2019_CVPR}. % for the use with graph-structured data.

\noindent{\textbf{Self-supervised learning}} leverages 
% easy-to-obtain auxiliary labels from spatial transformations \eg, rotations, patch permutations, contrast augmentation %and temporal steps 
% \etc, 
free supervision signals residing in images and videos
to promote robust representation learning in image recognition  \cite{dosovitskiy2014discriminative,doersch2015unsupervised,gidaris2018unsupervised}, video recognition \cite{fernando2017self,sermanet2017time,gan2018geometry}, video object segmentation~\cite{lai2020mast,zhu2020self}
and few-shot image classification \cite{gidaris2019boosting,su2019boosting}. 
Approaches \cite{gidaris2018unsupervised,doersch2015unsupervised,dosovitskiy2014discriminative} learn to predict random image rotations, relative pixel positions, and surrogate classes, respectively. Finally, \cite{gidaris2019boosting,su2019boosting} improve few-shot results by predicting image rotations/jigsaw patterns. 

\noindent{\textbf{Second-order statistics}} are used by us for permutation-invariant pooling. They
%
are also used for texture recognition \cite{tuzel_rc,elbcm_brod} by so-called Region Covariance Descriptors (RCD), object and action recognition \cite{koniusz2017higher,lei_beycov,pk_tpami_ar}. 
%A recent approach \cite{deep_cooc} extracts feature vectors at two separate locations in feature maps and performs an outer product to form a CNN co-occurrence layer. 
Second-order pooling has also been used in fine-grained image classification \cite{koniusz2018deeper,DeepKSPD,lei_beycov}, domain adaptation \cite{koniusz2017domain} and the fine-grained few-shot learning \cite{zhang2019power,wertheimer2019few,pk_hz_tpami_fsl}.

\noindent{\textbf{Few-shot action recognition}} %\cite{mishra2018generative,guo2018neural,xu2018dense,Zhu_2018_ECCV,dwivedi2019protogan} is a relatively new problem. A
approaches \cite{mishra2018generative,guo2018neural,xu2018dense} use a generative model, graph matching on 3D coordinates and a dilated networks with class-wise classifiers, respectively. Approach \cite{Zhu_2018_ECCV} proposes a so-called compound memory network using key-value memory associations. %for few-shot video classification. 
ProtoGAN \cite{dwivedi2019protogan} proposes a GAN model to generate action prototypes to address few-shot action recognition.

\subsection{Contrast with existing works}
\label{sec:contrast}
%
%Our model differs from existing few-shot action recognition methods in several aspects. 
Unlike  \cite{guo2018neural}, we use video clips rather than 3D skeletal coordinates. In contrast to \cite{xu2018dense}, we use relation/similarity learning and our training/testing class concepts are disjoint. While \cite{Zhu_2018_ECCV} memorizes  key values/frames, we model short- and long-term dependencies. %to attain robustness to the distribution shift of temporal discriminative blocks. 
While \cite{dwivedi2019protogan} forms action prototypes by GAN, we focus on self-supervised attention learning and permutation-invariant aggregation.

In contrast to self-supervision by rotations and jigsaw \cite{gidaris2019boosting,su2019boosting}, we use a sophisticated self-supervision on the attention unit for which a dedicated loss performs the alignment between the attention vector of augmented attention unit and the augmented in the same way attention vector from the non-augmented attention unit. Thus, we train a permutation-invariant attention to deal with the distribution shift of discriminative action locations.

%As second-order statistics are more informative than first-order average% pooling, 
Finally, we use second-order pooling \cite{koniusz2018deeper,zhang2019power}  for a permutation-invariant aggregation of temporal blocks while \cite{koniusz2018deeper,zhang2019power} work with images. We develop a theory explaining why Power Normalization helps episodic learning.



\subsection{Issues with fair comparisons}
\label{sec:issue}
%
Each few-shot action recognition method from Section \ref{sec:related} uses  different datasets and evaluation protocols making fair comparisons impossible. Class-wise splits/vali- dation sets are unavailable \ie, model \cite{mishra2018generative} uses a random split. Figures \ref{fig:ssta_loss}c and \ref{fig:ssta_loss}d of Section \ref{sec:exp} show that the random choice of the split set yields up to $\sim$6\% deviation in accuracy rendering such a protocol problematic. % (codes are not available either). %To compare our approach to prior work, we used the protocol of \cite{mishra2018generative} but we chose 5 splits at random to average results over multiple runs (we report an average-case not the best case results). We also used Kinetics split of \cite{Zhu_2018_ECCV}, and compared our approach with \cite{mishra2018generative,Zhu_2018_ECCV,dwivedi2019protogan}. 
%The above issues prompted us to
Thus, we propose a new protocol with class splits and validation sets made publicly available.

==> 3831 2/3-method.tex <==

\section{Approach}

\label{sec:approach}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/FSAR}
    \caption{\small Our few-shot Action Relation Network (ARN) contains: feature encoder with 4-layer 3D conv. blocks, relation network with 2D conv. blocks, and spatial and temporal attention units which refine the aggregation step. Specifically, we apply second-order pooling (operator $g$) over encoder outputs (re-weighted by attention vectors) per clip to obtain a Power Normalized Autocorrelation Matrix (AM). Query and support AMs per episode form relation descriptors (by operator $\vartheta$) from which the relation network learns to capture relations. The block (blue dashed line) is the self-supervised learning module which encourages our pipeline to learn auxiliary tasks \eg, {\em jigsaws}, {\em rotations}.}
    \label{fig:pipe}
\end{figure*}

\subsection{Pipeline}
%
Figure \ref{fig:pipe} shows our Action Relation Network (ARN). In contrast to the \textit{Conv-4-64} backbone in few-shot image classification  \cite{sung2017learning,zhang2019power,zhang2019few}, we adopt a C3D-based \textit{Conv-4-64} backbone to extract spatio-temporal features which capture short-range dependencies. Next, we apply second-order pooling on 3D action features re-weighted by attention to obtain second-order statistics which are permutation-invariant \cite{koniusz2018deeper} \wrt the spatio-temporal order of features. To paraphrase, we discard the long-range order of temporal (and spatial) blocks captured by the encoder. Finally, second-order matrices form relation descriptors from query/support clips fed into a 2D relation network to capture relations. % within so-called episodes \cite{sung2017learning}.

Let $\mathbf{V}$ denote a video (\ie, with $\sim\!$20 frames) and $\mPhi\!\in\!\mbr{C\times T\times H\times W}$ be features extracted from $\mathbf{V}$  by $f$:
\begin{equation}
    \mPhi = f(\mathbf{V}; \tF).
    \label{eq:enc}
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/attention-modules}
    \caption{\small Spatial and temporal units are shown in Fig. \ref{fig:ar_attention}a. A naive approach is to directly extract the temporal and spatial attention, whose size is $1\times T\times H\times W$. However, this is computationally expensive and results in overparametrization. Thus, we split the attention block into separate spatial and temporal branches whose impact is adjusted by $\alpha_s$ and $\alpha_t$. Fig. \ref{fig:ar_attention}b is the $\kappa$ ratio \wrt~the $Z$-shot value (see Eq. \eqref{eq:support}). The dashed curve shows that as $Z$ grows (0 denotes the regular classification), the memorization burden of co-occurrence $(i,j)$ on the comparator grows $\kappa$ times for second-order pooling without Power Normalization (as opposed to Power Normalization). The solid line shows that as we use larger $N$ (video clips \vs images), not using PN is even more detrimental.}
    \label{fig:ar_attention}
\end{figure}


%Then we vectorize $\mPhi$ to obtain $\mPhi\!\in\!\mbr{C\times THW}$, and apply second-order pooling to get the Second-order Pooling Matirx (SPM) representation $\mPsi\!\in\!\mbr{C\times C}$:

To aggregate $\mPhi$ per clip into $\mPsi$, we apply a pooling operator $g$ over the support and query features, resp. For $g$, we use pooling operators from Sec. \ref{sec:pool}:  

\begin{equation}
    \mPsi = g(\mPhi).
\end{equation}

Once $\mPsi$ are computed for query/support clips, they form relation descriptors (via operator $\vartheta$) passed to the relation network $r$ to obtain the relation score $\zeta_{sq}$:
%
\begin{equation}
    \zeta_{sq} = r(\vartheta(\mPsi_s, \mPsi_q); \tR),
\end{equation}
where $\tR$ are parameters of network $r$, and $\vartheta$ forms relation descriptors \eg, we use the concatenation along the channel mode.

We use the Mean Square Error (MSE) loss over support and query pairs:
\begin{equation}
    L = \sum\limits_{s\in S}\sum\limits_{q\in Q} (\zeta_{sq} - \delta(l_s-l_q))^2,
\end{equation}
where $\delta(l_s\!-\!l_q)\!=\!1$ if $l_s\!=\!l_q$, $\delta(l_s\!-\!l_q)\!=\!0$ otherwise. Class labels of support and query action clips are denoted as  $l_s$ and $l_q$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/ar-ss-attention}
    \caption{Augmentation-guided attention by alignment. We firstly collect the encoded representations of original and augmented data, then we extract the temporal or spatial attention vectors from them. We apply the same augmentation(s) on the temporal or spatial attention vectors of the original data resulting in the augmented attention vectors which we align with attention vectors of the augmented data.}
    \label{fig:ss_attention}
\end{figure*}

\subsection{Pooling of encoded representations}
\label{sec:pool}
For permutation-invariant pooling of temporal (and spatial) blocks, we investigate three pooling mechanisms discussed below.

\noindent{\textbf{Average and max pooling}} are two widely-used pooling functions which can be used for aggregation of $N\!=\!T\!\times\!W\!\times\!H$ fibers (channel-wise vectors) of feature map $\mPhi$ defined in Eq. \eqref{eq:enc}. The average pooling is given as $\vpsi\!=\! \frac{1}{N}\sum_{n=1}^N\vphi_n$ where $\vpsi\!\in\!\mbr{C}$, and $\vphi_n\!\in\!\mbr{C}$ are $N$ fibers. Similarly, max pooling is given by $\psi_c\!=\!\!\! \max\limits_{n=1,\cdots,N}\phi_{cn},\, c\!=\!1,\cdots,C$, and $\vpsi=[\psi_1,\cdots,\psi_C]^T$. Average and max pooling are commutative \wrt~the input fibers, thus being permutation-invariant. However, first-order pooling is less informative than second-order \cite{koniusz2016tensor} discussed next.

\noindent{\textbf{Second-order pooling}} captures correlations (or co-occurrences) between pairs of features in $N$ fibres of feature map $\mPhi$, which is reshaped such that $\mPhi\in\mbr{C\times N}$, $N=T\times H\times W$. Such an operator proved robust in classification \cite{koniusz2016tensor} and  few-shot learning \cite{zhang2019power,wertheimer2019few,pk_hz_tpami_fsl}. %Below we demonstrate that how we apply co-occurrence pooling over 3D convolutional action features.
%
Specifically, we define:
%
%
%
\begin{align}
& \!\!\!\mPsi=\eta\Big(\frac{1}{N}\sum_{n=1}^N\!\vphi_n\vphi_n^T\Big)=\eta\Big(\frac{1}{N}\mPhi\mPhi^T\Big)\quad\text{where}\quad\eta(\mX) = \frac{1 - \exp({\sigma \mX})}{1 + \exp({\sigma \mX})}.\label{eq:hok3}
\end{align}
%\vspace{-0.2cm}
%
%

\noindent{Matrix} $\mPsi\in\mbr{C\times C}$ is a Power Normalized autocorrelation matrix capturing correlations of fiber features $\vphi_n$ of feature map $\mPhi$ from Eq. \eqref{eq:enc} while $\eta$ applies Power Normalization (PN): we use the zero-centered element-wise Sigmoid \cite{koniusz2016tensor,zhang2019power} on $\mX$, and
%
%\begin{align}
%    \eta(\mX) = \frac{1 - \exp({\sigma \mX})}{1 + \exp({\sigma \mX})},
%\end{align}
 $\sigma$ controls the slope of PN. For a given pair of features $i$ and $j$ in matrix $\mPsi$, that is $\Psi_{ij}$, the role of PN is to  detect the likelihood if at least one co-occurrence of features $i$ and $j$ has been detected \cite{koniusz2016tensor}.
%------------------------------------------------------------------------- 
%
According to Eq. \eqref{eq:hok3}, second-order pooling is permutation-invariant \wrt~the order of input fibers as the summation in Eq. \eqref{eq:hok3} is commutative \wrt~the order of $\vphi_1,\cdots,\vphi_N$. Thus, second-order pooling factors out the spatial and temporal modes of $\mPhi$ and aggregates clips with varying numbers of temporal blocks (discards the order of long-range spatial/temporal dependencies) into a fixed length representation $\mPsi\in\mbr{C\times C}$. Below we explain further why second-order pooling with Power Normalization is  well suited for episodic few-shot learning.

\noindent{\textbf{Relation descriptors}} between query/support pooled matrices $\mPsi_q$ and $\mPsi_s$ are formed by operation $\vartheta(\mPsi_q,\mPsi_s)$ which, in our case, simply performs concatenation of $\mPsi_q$ with $\mPsi_s$ along the channel mode by $\text{cat}(\mPsi_q, \mPsi_s)\in\mbr{2\times C\times C}$, and $\mPsi_s$ is obtained by the mean (or maximum) along the channel mode between $\mPsi_s^{1},\cdots,\mPsi_s^{Z}$  belonging to the same episode and class ($Z\!>\!1$ for the few-shot case).

It is known from \cite{koniusz2018deeper} that the Power Normalization in Eq. \eqref{eq:hok3} performs a co-occurrence detection rather than counting (correlation). For classification problems, assume a probability mass function $p_{X_{ij}}(x)\!=\!1/(N\!+\!1)$ if $x\!=\!0,\cdots,N$, $p_{X_{ij}}(x)\!=\!0$ otherwise, that tells the probability that co-occurrence between $\Phi_{in}$ and $\Phi_{jn}$ happened $x\!=\!0,\cdots,N$ times (given some clip). Note that  classification often  depends on detecting a co-occurrence (\eg, is there a flower co-occurring with a pot?) rather than counts (\eg, how many flowers and pots co-occur?). Using second-order pooling without PN requires a classifier to observe $N\!+\!1$ training samples of {\em flower and pot} co-occurring in quantities $0,\cdots,N$ to memorise all possible co-occurrence count configurations. For relation learning, our $\vartheta$ stacks pairs of samples to compare, thus a comparator now has to deal with a probability mass function of ${R_{ij}}\!=\!{X_{ij}}\!+\!{Y_{ij}}$ depicting {\em flowers and pots} whose  $\text{support}(p_{R_{ij}})\!=\!2N\!+\!1\!>\!\text{support}(p_{X_{ij}})\!=\!N\!+\!1$ if random variable $X\!=\!Y$ (same class). The same is shown by variances  $\text{var}(p_{R_{ij}})\!>\!\text{var}(p_{X_{ij}})$. For $Z$-shot learning, the growth of variance and support equal $(Z\!+\!1)N\!+\!1$  indicates that the comparator has to memorize more configurations of co-occurrence $(i,j)$ as $Z$ grows.

However, this situation is alleviated by Power Normalization (operator $\eta$) whose  probability mass function can be modeled as $p_{X^\eta_{ij}}(x)\!=\!1/2$ if $x\!=\!\{0,1\}$, $p_{X^\eta_{ij}}(x)\!=\!0$ otherwise, as PN detects a co-occurrence (or its lack). For $Z$-shot learning, $\text{support}(p_{R^\eta_{ij}})\!=\!Z\!+\!2\!\ll\!\text{support}(p_{R_{ij}})\!=\!(Z\!+\!1)N\!+\!1$. The  ratio given as
%
\begin{align}
\kappa\!=\!\frac{\text{support}(p_{R_{ij}})}{\text{support}(p_{R^\eta_{ij}})}\!=\!\frac{(Z\!+\!1)N\!+\!1}{Z\!+\!2}
\label{eq:support}
\end{align}

\noindent{shows} that the comparator has to memorize many more count configurations of co-occurrence $(i,j)$ for naive pooling compared to PN as $Z$ and/or $N$ grow ($N$ depends on the number of temporal and spatial blocks $T$, $H$ and $W$). Figure \ref{fig:ar_attention} shows how $\kappa$ varies \wrt~$Z$ and $N$. Our modeling assumptions are simple \eg, the assumption on mass functions with uniform probabilities, the use of the support of mass functions rather than variances to describe variability of co-occurrence $(i,j)$. Yet, substituting these modeling choices with more sophisticated ones does not affect  theoretical conclusions that: (i) PN benefits few-shot learning ($Z\!\geq\!1$) more than the regular classification ($Z\!=\!0$) in terms of reducing possible count configurations of $(i,j)$, and (ii) for videos (large $N$) PN reduces the number of count configurations of $(i,j)$ more rapidly than for images (smaller $N$). While classifiers and comparators do not learn exhaustively all count configurations of co-occurrence $(i,j)$ as they have some generalization ability, they learn quicker and better if the number of count configurations of $(i,j)$ is limited. % in the low-sample learning regime.

\subsection{Temporal and spatial attention}
Figure \ref{fig:ar_attention}a introduces decoupled spatial/temporal attention units consisting of three 3D Convolutional blocks and a Sigmoid output layer. Let $t$ and $s$ denote the temporal and spatial attention modules, and  the attention be applied ahead of second-order pooling. We obtain temporal and spatial attention maps  $\mathbf{T}\in\mbr{1\times T\times 1\times 1}$ and  $\mathbf{S}\in\mbr{1\times 1\times \times H\times W}$, and attentive action features $\mPhi^*$ by:
\begin{align}
    \mathbf{T} = t(\mPhi; \tT), \;\mathbf{S} = s(\mPhi; \tS), \\
    \mPhi^* = (\alpha_t + \mathbf{T})\cdot(\alpha_s +\mathbf{S})\cdot\mPhi,\label{eq:sh}
\end{align}
where $\tT$ and $\tS$ are network parameters of temporal/spatial attention units while $\alpha_t$ and $\alpha_s$ control the impact of attention vectors.

Using attention helps spot discriminative temporal/spatial blocks, and suppress uninformative regions. However, the attention  should be robust to varying distributions of locations of discriminative blocks in clips as proposed below.
%invariant to data augmentations e. g., spatial rotation and jigsaw, temporal shuffling, \textit{et al}, thus assuring the expected key frames and regions are accurately localized for relation learning. However, using attention in the above naive way cannot assure this important property, %on produced temporal and spatial localizing attention maps,
%thus we propose to encourage such a property via self-supervision, which is detailed in the following section.

%\vspace{-0.3cm}
\subsection{Temporal and spatial self-supervision}
Self-supervised Learning (SsL) helps %to co-regularize a network  and improve classification results.
learn representations without using manually-labeled annotations. % for supervision. 
%In contrast to previous papers on self-supervised learning, 
We  impose self-supervision both on encoders and attention units. % to %fully address the domain shift issue and 
%enhance the robustness against augmentations. %Combining self-supervision with the attention mechanism in a few-shot learning pipeline is a `kill two birds with one stone' type of design which simultaneously enriches the patterns of training samples and effectively improves the robustness of attentions. 
 % mechanisms to co-regularize the feature encoder and attention units.
%
%We start with self-supervision via augmentation tasks. % related in some way to the main classification task. %These properties make it fit few-shot learning well. %To effectively enrich temporal and spatial patterns of training action clips and form better understanding of various actions, the common ways are shuffling the temporal orders with different random seeds, spatially rotating images with specific degrees or applying jigsaw patterns. 
For temporal self-supervision, we augment clips by shuffling the order of temporal blocks, which primes our network to become robust to long-term non-repetitive temporal dependencies in clips. Self-supervision also helps overcome the low-sample %regime of few-shot learning
by encouraging network to learn  auxiliary tasks. In contrast, previous works %on self-supervision in action recognition 
shuffled frames which breaks the highly discriminative short-term temporal dependencies. %Thus, we propose a novel temporal shuffling strategy, namely a temporal jigsaw. For the spatial self-supervision, we apply the standard random rotations and random jigsaw permutations. 
We use the following self-supervision strategies:
%
%Below we demonstrate different types of temporal and spatial self-supervision used in our paper:
\renewcommand{\labelenumi}{\roman{enumi}.}
\begin{enumerate}[leftmargin=0.6cm]
    \item \textbf{Temporal jigsaw.} Jigsaw, a popular self-supervisory task breaks the object location bias and teaches the network to recognize shuffling. As in \cite{Xu_2019_CVPR}, we split clips into non-overlapping fixed-length temporal blocks and shuffle them. %Thus, we break up long-term temporal patterns which are unlike to repeat in videos. % but we preserve shorter discriminative  patterns to attain a local action consistency.
    \item \textbf{Spatial jigsaw.} We split frames into four non-overlapping regions, then randomly permute them.
    \item \textbf{Rotation.} As the most popular self-supervisory task are rotations, we uniformly rotate all frames per clip by a random angle ($0^{\circ}$, $90^{\circ}$, $180^{\circ}$, $270^{\circ}$).
\end{enumerate}

%Similarly to other works on self-supervised learning, we employ
Figure \ref{fig:pipe} (blue frame) shows how we apply and recognize the self-supervision patterns \eg, shuffling and rotation angles. %Introducing such auxiliary tasks  is the  strategy underlying self-supervision  which we use in this paper. 
%
Below, we illustrate self-supervision via  rotations. Consider the objective function $L_{rot}$ for self-supervised learning with a self-supervision discriminator $d$, where $\tD$ are parameters of $d$. Thus:
\begin{align}
   & \hat{\mPhi}_i = f(\;rot(\mathbf{V}_i, \theta)\; ;\tF), \\
&\mathbf{p}_{rot_i} = d(\hat{\mPhi_i}; \tD),\\
%\end{align}
%
%\begin{equation}
   & \!\!\!\!\!\!\!\!\!\!\!\!\!L_{rot} = - \sum\limits_{i} log\left(\frac{\exp({\mathbf{p}_{rot_{i}}[l_{\theta i}]})}{\sum_{s}\exp({\mathbf{p}_{rot_{i}}\![l_{s}]})}\right),
    \label{eq:ssrot}
\end{align}
%\end{equation}
%
%
where $\mathbf{V}_i$ is a randomly sampled clip, $\theta\in\{0\degree, 90\degree, 180\degree, 270\degree\}$ is a randomly selected rotation angle of a frame, $l_{\theta_i}\!\in\!\{0,1,2,3\}$ is the rot. label for sample $i$.

Combining the original loss function $L$ with such a self-supervision term $L_{rot}$ results in a self-supervised few-shot action recognition pipeline. However, this objective does not make the attention to be invariant to augmentations per se.

\subsection{Augmentation-guided attention by alignment}
%
Figure \ref{fig:ss_attention} presents a strategy in which we extract the attention vector for an augmented  clip, then we apply  the same augmentation to the attention vector obtained from the original non-augmented clip, and we encourage such a pair of augmentation vectors to align by a dedicated MSE loss. This encourages the attention unit to be invariant \wrt~a given augmentation type. Fig. \ref{fig:demo}a explains why the temporal permutation strategy  benefits few-shot learning while Figure \ref{fig:ss_attention} shows how to apply permutations and rotations.
%
As an example, for a rotation-guided spatial-attention we define the alignment loss $L_{att}$:
%
\begin{align}
\hat{\vPhi_i} & = f(\;rot(\mathbf{V}_i, \theta)\; ;\tF),  \\
S_i & = s(\vPhi_i; \tS), \; \hat{S}_i  = s(\hat{\vPhi}_i; \tS), \\
L_{att} & = \;\sum\limits_{i}\;||\;|\;rot(S_i, \theta) - \hat{S}_i\;| - \lambda \;||^2_F. %& - \eta(\parallel S \parallel^2_2 + \parallel \hat{S} \parallel^2_2).
\end{align}
%
\noindent{where} $\lambda$  controls the strictness of alignment. The final objective then becomes:
%
\begin{equation}
    %\min
    \argmin\limits_{\tF, \tD, \tT, \tS}\quad L + \beta L_{ss} + \gamma L_{att}
    \label{eq:finloss}
\end{equation}
where $\beta$ and $\gamma$ are the hyper-parameters adjusted by cross-validation, $L_{ss}$ is a chosen type of self-supervision \eg, via rotations as introduced in Eq. \eqref{eq:ssrot}.






==> 3831 2/4-experiments.tex <==

\section{Experiments}
\label{sec:exp}
% Below we demonstrate our experimental setup and detailed evaluation results.
\subsection{Experimental setup}
%Each of prior few-shot action recognition papers in the literature use different evaluation protocols, which makes it difficult if not impossible to conduct a fair comparison, Thus, we hope to standardize few-shot training, validation, and test splits for several classic action recognition benchmarks. 
Below, we describe our setup and evaluations in detail. To exclude  complicated data pre-processing and frame sampling steps typically used in action recognition, we sample uniformly 20 frames along the temporal mode for each dataset. % and apply mean-std normalize on them.

\begin{table*}[t]
\caption{Comparisons between our ARN model and existing works on HMDA51 and UCF101 splits proposed in \cite{mishra2018generative} and a Kinetics split from \cite{Zhu_2018_ECCV} (given 5-way acc.)}
\label{tab:compar}
\makebox[\textwidth]{
\setlength{\tabcolsep}{0.4em}
%\renewcommand{\arraystretch}{0.90}
\fontsize{9}{10}\selectfont
\begin{tabular}{l|cccccc}
\toprule
\multirow{2}{*}{$\;\;\;\;\;\;$Model} & \multicolumn{2}{c}{HMDB51 \cite{mishra2018generative}} & \multicolumn{2}{c}{UCF101 \cite{mishra2018generative}} & \multicolumn{2}{c}{Kinetics \cite{dwivedi2019protogan}} \\
 & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
\textit{GenApp} $\;\;\;\;$\cite{mishra2018generative} & ${- }$ & ${52.5 \pm 3.10}$ & ${-}$ & ${78.6 \pm 2.1}$ & - & - \\
\textit{ProtoGAN} \cite{dwivedi2019protogan} & $34.7 \pm 9.20 $ & $54.0 \pm 3.90$ & $57.8 \pm 3.0$ & $80.2 \pm 1.3$ & - & - \\
\textit{CMN} $\;\;\;\;\;\;\;\;$\cite{Zhu_2018_ECCV} & - & - & - & - & 60.5 & 78.9 \\
\hline
\textit{Ours} & $\mathbf{44.6 \pm 0.9}$ & $\mathbf{59.1 \pm 0.8}$ & $\mathbf{62.1 \pm 1.0}$ & $\mathbf{84.8 \pm 0.8}$ & $\mathbf{63.7}$ & $\mathbf{82.4}$ \\
\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[t]
\centering
\caption{Ablations of different modules of ARN given our proposed HMDB51 protocol (given 5-way acc.) We used {\em spatial-jigsaw} for self-supervision.}
\label{tab:att}
\makebox[\textwidth]{
\setlength{\tabcolsep}{0.4em}
%\renewcommand{\arraystretch}{0.90}
\fontsize{9}{7}\selectfont
\begin{tabular}{cccc|cc}
\toprule
Baseline & Spatial Attention & Self-supervision  & Alignment & 1-shot & 5-shot \\
\hline
\checkmark & & & & 40.83 & 55.18 \\
\checkmark & \checkmark & & & 41.27 & 56.12 \\
\checkmark & & \checkmark & & 44.19 & 58.50 \\
\checkmark & \checkmark & \checkmark & & 44.61 & 59.71 \\
\checkmark & \checkmark &  & \checkmark & 43.11 & 57.35 \\
\checkmark & \checkmark & \checkmark & \checkmark & \textbf{45.17} & \textbf{60.56}  \\
\bottomrule
\end{tabular}}
\end{table*}

\vspace{0.05cm}
\noindent\textbf{HMDB51} \cite{Kuehne11}  contains 6849 clips divided into 51 action categories, each with at least 101 clips, 
31, 10 and 10 classes selected for training,  validation and  testing.

\noindent\textbf{Mini Moments in Time (miniMIT)} \cite{monfortmoments} %is a subset of the newly proposed large-scale Moments in Time (MIT) dataset. The mini version, suitable for few-shot learning, 
contains 200 classes and 550 videos per class. We select 120, 40 and 40 classes for training, validation and testing.

\noindent\textbf{UCF101} \cite{soomro2012ucf101}, action videos from Youtube, has 13320 video clips and 101 action classes. We randomly select 70 training, 10 validation and 21 testing classes. 

\noindent\textbf{Kinetics}, used by  \cite{Zhu_2018_ECCV} to select a subset  for few-shot learning, consists of  64, 12 and 24 training, validation and testing classes. We use it for comparisons.

Training, validation and testing splits on the first three datasets are detailed in our supplementary material while authors of \cite{Zhu_2018_ECCV} provide the split on Kinetics. 
The frames of action clips from all  datasets are resized to $128\times128$. All models are trained on training splits. Validation set is only used for cross-validation. %to search for the optimal hyper-parameters, while the test set is used for evaluations only.


\begin{table*}[t]
\centering
\caption{Evaluations on HMDB51 (5-way acc.) Attention: Temporal (TA), Spatial (SA). Self-super.: Temp. (TS), Spat. (SS), Self-Super. \& Alignment: Temp. (TSA), Spat. (SSA).$\!\!\!\!$}
\label{tab:1}
\makebox[\textwidth]{
\setlength{\tabcolsep}{1.2em}
%\renewcommand{\arraystretch}{0.90}
\fontsize{10}{12}\selectfont
\begin{tabular}{lcc}
\toprule
Model & 1-shot & 5-shot  \\
\hline
& \multicolumn{2}{c}{Baseline} \\
\hline
\textit{C3D Prototypical Net} \cite{snell2017prototypical} & ${38.05 \pm 0.89}$ & ${53.15 \pm 0.90}$\\
\textit{C3D RelationNet} \cite{sung2017learning}  & ${38.23 \pm 0.97}$ & ${53.17 \pm 0.86}$\\
\textit{C3D SoSN} \cite{zhang2019power}  & ${40.83 \pm 0.96}$ & ${55.18 \pm 0.86}$\\
%\textit{C3D SoSN-new} \cite{zhang2019power} & $43.02 \pm 0.99$ & $56.48 \pm 0.88$ \\
\hline
 \multicolumn{3}{c}{ \bf Temporal/Spatial Attention only (TA \vs~SA)} \\
\hline
\textit{ARN+TA}  & ${41.97 \pm 0.97}$ & ${57.67 \pm 0.88}$\\ %57.24
\textit{ARN+SA}  & ${41.27 \pm 0.98}$ & ${56.12 \pm 0.89}$\\
\textit{ARN+SA+TA}  & ${42.41 \pm 0.99}$ & ${56.81 \pm 0.87}$\\
\hline
\multicolumn{3}{c}{\bf Temporal/Spatial Self-supervision only (TS \vs~SS)} \\
\hline
\textit{ARN+TS (temp. jigsaw)}  & ${43.79 \pm 0.96}$ & ${58.13 \pm 0.88}$\\
\textit{ARN+SS (spat. jigsaw)}  & ${44.19 \pm 0.96}$ & ${58.50 \pm 0.86}$\\
\textit{ARN+SS (rotation)}  & ${43.90 \pm 0.92}$ & ${57.20 \pm 0.90}$\\
\hline
\multicolumn{3}{c}{\bf Temp./Spat. Self-super. \& Att. by alignment (TSA\! \vs~\!SSA)} \\
%& \multicolumn{2}{c}{\bf $\!\!\!\!\!\!\!\!\!\!\!\!\!\!$Temporal/Spatial Attention Units+SS+A} \\
\hline
%\textit{ARN+SA (spatial-jigsaw)}  & ${45.15 \pm 0.96}$ & ${60.56 \pm 0.86}$\\
%\textit{ARN+SA (rotation)}  & ${45.52 \pm 0.96}$ & ${58.96 \pm 0.87}$\\ 
%\textit{ARN+TA (temporal-jigsaw)}  & ${45.20 \pm 0.98}$ & ${59.11 \pm 0.86}$\\
%\textit{ARN+SA+TA (all)} &  $\mathbf{46.13 \pm 0.95}$ & $\mathbf{60.92 \pm 0.86}$\\
\textit{ARN+TSA (temp. jigsaw)}  & ${45.20 \pm 0.98}$ & ${59.11 \pm 0.86}$\\
\textit{ARN+SSA (spat. jigsaw)}  & ${45.15 \pm 0.96}$ & ${60.56 \pm 0.86}$\\
\textit{ARN+SSA (rotation)}  & ${45.52 \pm 0.96}$ & ${58.96 \pm 0.87}$\\ 

%\textit{ARN+TSA+SSA} &  $\mathbf{46.13 \pm 0.95}$ & $\mathbf{60.92 \pm 0.86}$\\
\bottomrule
\end{tabular}}
\end{table*}




\begin{table*}[t]
\centering
\caption{Evaluations on \textit{mini}MIT and UCF101 datasets (given 5-way acc.) See the legend at the top of Table \ref{tab:1} for the description of abbreviations.}
\label{tab:2}
\makebox[\textwidth]{
\setlength{\tabcolsep}{0.4em}
%\renewcommand{\arraystretch}{0.90}
\fontsize{9}{12}\selectfont
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{miniMIT} & \multicolumn{2}{c}{UCF101} \\
Model & 1-shot & 5-shot & 1-shot & 5-shot \\ \hline
\textit{C3D Prototypical Net} \cite{snell2017prototypical} & ${33.65 \pm 1.01}$ & ${45.11 \pm 0.90}$ & ${57.05 \pm 1.02}$ & ${78.25 \pm 0.73}$\\
\textit{C3D RelationNet} \cite{sung2017learning} & ${35.71 \pm 1.02}$ & ${47.32 \pm 0.91}$ & ${58.21 \pm 1.02}$ & ${78.35 \pm 0.72}$\\
\textit{C3D SoSN} \cite{zhang2019power} & $40.83 \pm 0.99$ & $52.16 \pm 0.95$ & $62.57 \pm 1.03$ & $81.51 \pm 0.74$\\
\hline
\multicolumn{5}{c}{\bf Temporal/Spatial Attention only (TA \vs~SA)} \\
\hline
\textit{ARN+TA} & ${41.65 \pm 0.97}$ & ${56.75 \pm 0.93}$ & ${63.35 \pm 1.03}$ & ${80.59 \pm 0.77}$\\
\textit{ARN+SA} & ${41.27 \pm 0.98}$ & ${55.69 \pm 0.92}$ & ${63.73  \pm 1.08}$ & ${82.19 \pm 0.70}$\\
\textit{ARN+TA+SA} & ${41.85 \pm 0.99}$ & ${56.43 \pm 0.87}$ & ${64.48 \pm 1.06}$ & ${82.37 \pm 0.72}$\\
\hline
\multicolumn{5}{c}{\bf Temporal/Spatial Self-supervision only (TS \vs~SS)} \\
\hline
\textit{ARN+TS (temp. jigsaw)} &  ${42.45 \pm 0.96}$ & ${54.67 \pm 0.87}$ &  ${63.79 \pm 1.02}$ & ${82.14 \pm 0.77}$\\
\textit{ARN+SS (spat. jigsaw)} & ${42.68 \pm 0.95}$ & ${54.46 \pm 0.88}$ &  ${63.75 \pm 0.98}$ & ${80.92 \pm 0.72}$\\
\textit{ARN+SS (rotation)} & ${42.01 \pm 0.94}$ & ${56.83 \pm 0.86}$ &  ${63.95 \pm 1.03}$ & ${81.09 \pm 0.76}$\\
\hline
\multicolumn{5}{c}{\bf Temp./Spat. Self-super. \& Att. by alignment (TSA\! \vs~\!SSA)} \\
\hline
\textit{ARN+TSA (temp. jigsaw)} & ${42.65 \pm 0.94}$ & ${57.35 \pm 0.85}$ & ${65.46 \pm 1.05}$ & ${82.97 \pm 0.71}$\\
\textit{ARN+SSA (spat. jigsaw)} & ${42.92 \pm 0.95}$ & ${56.21 \pm 0.85}$ & ${66.04 \pm 1.01}$ & ${82.68 \pm 0.72}$\\
\textit{ARN+SSA (rotation)} & ${43.05\pm 0.97}$ & ${56.71 \pm 0.87}$ & ${66.32 \pm 0.99}$ & ${83.12 \pm 0.70}$\\
%\textit{ARN+TSA+SSA} & $\mathbf{43.61 \pm 0.96}$ & $\mathbf{58.12 \pm 0.84}$ & $\mathbf{66.98 \pm 1.02}$ & $\mathbf{84.25 \pm 0.73}$\\
\bottomrule
\end{tabular}}
\end{table*}

\subsection{Comparison with previous works}
\label{sec:weak}

Section \ref{sec:issue} explains the issues with existing methods, protocols, and the lack of publicly available codes. %However, we strive for a fair  comparison of our approach to other methods. 
For a fair comparison, we use firstly the protocol of \cite{mishra2018generative} (HMDB51 and UCF101 datasets) but we chose 5 splits at random according to their protocol to average results over multiple runs: we report an average-case result not the best case or a single run result (in contrast to \cite{mishra2018generative}). We also use the Kinetics split of \cite{Zhu_2018_ECCV}, and compare our approach with \cite{mishra2018generative,Zhu_2018_ECCV,dwivedi2019protogan}. 

Table \ref{tab:compar} shows that our ARN (best variant) outperforms GenApp \cite{mishra2018generative}, ProtoGAN \cite{dwivedi2019protogan}, CMN \cite{Zhu_2018_ECCV} by a large margin of 3\% to 10\% on the three protocols.  Our standard errors are low as they result from  5 runs on 5 splits (average case) while a large deviation of ProtoGAN \cite{dwivedi2019protogan} was obtained \wrt~episodes on a single split.

\vspace{0.05cm}
\noindent\textbf{The weakness of  protocol \cite{mishra2018generative}.} Evaluation protocols in \cite{mishra2018generative} rely on randomly selecting training/testing classes with 50--50 ratio from all classes to form  training/testing splits on HMDB51 and UCF101. The performance of that protocol varies heavily due to the randomness. Moreover, results of \cite{mishra2018generative} are reported on a single run. % and the code is not given. 
Figures \ref{fig:ssta_loss}c and  \ref{fig:ssta_loss}d show up to 6\% variations due to the randomness, making a fair comparison between models difficult on such a protocol. The lack of validation set makes cross-validation also a random process affecting results.

We rectify all this by providing standardized training, validation, and testing splits on HMDB51, \textit{mini}MIT and UCF101.  In what follows, we use our new splits with our few-shot ARN. 
%
We equip the Prototypical Net \cite{snell2017prototypical}, Relation Net \cite{sung2017learning} and SoSN \cite{zhang2019power} with a 3D conv. feature encoder ({\em C3D}) for baselines used below. 

\vspace{0.05cm}
\noindent\textbf{ARN modules (ablations).}  We start by studying ARN modules on HMDB51. %to establish their impact on results. 
Table \ref{tab:att} shows that combining attention with the baseline C3D SoSN pipeline brings $\sim$1\% gain. Switching to the attention by alignment brings 1.2--1.9\% gain over  the naive attention unit. Combining self-supervision with (i) the baseline and (ii) the baseline with attention brings $\sim$3\% and $\sim$3.5\% gain, resp. Combining all units together (attention, self-supervision and alignment) yields $\sim$\textbf{5}\% gain. The  computational cost is %(combination of loss functions) 
similar to running either self-supervision or alignment.

Thus, in what follows we will report results for the most distinct four variants: (i) baseline ({\em C3D SoSN}), (ii) Temporal/Spatial Attention only ({\em TA} \& {\em SA}), Temporal/Spatial Self-supervision w/o attention ({\em TS} \& {\em SS}), and Temporal/Spatial Self-supervision with attention by alignment ({\em TSA} \& {\em SSA}). 


\begin{table*}[b]
\centering
\caption{\small Comparison of pooling functions on our HMDB51 split (5-way 1-shot).}
\label{tab:pooling}
\makebox[\textwidth]{
\setlength{\tabcolsep}{0.3em}
%\renewcommand{\arraystretch}{0.90}
\fontsize{8}{10}\selectfont
\begin{tabular}{cccccc}
\toprule
No Pooling & Average & Average+PN & Max & Second-order (w/o PN) & Second-order (with PN) \\ \hline
35.71 & 39.51 & 40.02 & 38.95 & 39.97 & $\mathbf{40.83}$ \\
\bottomrule
\end{tabular}}
\end{table*}

\noindent\textbf{Pooling (ablations).} Section \ref{sec:pool} discusses pooling variants from Table \ref{tab:pooling}. Second-order pooling (with PN) outperforms second-order pooling (w/o PN) followed by average and max pooling. Combining average pooling with PN boosts its results which is consistent with the theoretical analysis in Figure \ref{fig:ar_attention}. In what follows, we use the best pooling variant only, that is second-order pooling with PN.

\noindent\textbf{Main evaluations.} Tables \ref{tab:1} and \ref{tab:2} present main evaluations on the proposed by us protocols. Notably, our approaches outperform all baselines (known approaches enhanced by us with the  C3D-based encoder). Below, we detail the results.

\noindent\textbf{Attention.} Tables \ref{tab:1} and  \ref{tab:2} investigate the Temporal and Spatial Attention denoted as ({\em TA}) and  ({\em SA}) on our few-shot ARN. TA on the 1-shot and 5-shot protocols improves the accuracy by $1.0\%$ and $2.5\%$ while SA boosts the 1- and 5-shot accuracy by $0.5\%$ and $1.0\%$, respectively. 
%
For the combined Temporal and Spatial Attention ({\em TA}+{\em SA}), the  Eq. \eqref{eq:sh} is used with  $\alpha_s\!=\!1.0$ and $\alpha_t\!=\!0.5$ (HMDB51) and $\alpha_s\!=\!1.5$ and $\alpha_t\!=\!1.0$ (UCF101) chosen on the validation split. %to obtain strong performance, however, it still requires cross-validation on the two parameters to achieve the best performance.
Tables \ref{tab:1} and  \ref{tab:2} show that
SA+TA  achieves a further improvement of up to $1.1\%$ for 1-shot learning but for 5-shot learning it may suffer an $0.8\%$ drop in accuracy compared to the best score of TA and SA while still achieving between an 0.8 and 4.2\% gain over the baseline  C3D SoSN. This  is consistent with our argument that vanilla attention units can be further improved for a better performance. 

\noindent\textbf{Temporal/spatial self-supervision.} In this experiment, we disable attention units. Tables \ref{tab:1} and  \ref{tab:2} show that self-supervision \wrt~either temporal or spatial mode boosts performance of 1-shot and 5-shot learning over the  C3D SoSN baseline on HMDB51 up to 3.2\%. On miniMIT, we observe gains between 1.2 and 4.6\%. On UCF101, we see gains between 0.6 and 1.4\%. However, for UCF101 dataset, self-supervision by the spatial jigsaw and rotation lead to a marginal performance drop on 5-shot learning compared to  C3D SoSN. %As videos from UCF101 often share some common properties, such as similar background, similar viewpoint, similar centering of the subject within frames, \etc, we expect that spatial auxiliary tasks cannot help boost the results on the data where spatial properties are fixed.



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/loss-old-splits}
    %\vspace{-0.7cm}
    \caption{\small In Fig. \ref{fig:ssta_loss}a are the loss curves for Eq. \eqref{eq:finloss}. Fig. \ref{fig:ssta_loss}b shows the validation score \wrt~$\gamma$ (1-shot prot.) Applying Spatial Self-super. \& Attention by alignment (SSA) $\gamma\!>\!0$ outperforms the Spatial Self-super. \& Attention only ($\gamma\!=\!0$). Fig. \ref{fig:ssta_loss}c and \ref{fig:ssta_loss}d show the performance variation on random splits of HMDB51 and UCF101 proposed by \cite{mishra2018generative}.}
    %\vspace{-0.4cm}
    \label{fig:ssta_loss}
\end{figure}

\noindent\textbf{Temporal/spatial self-supervision \& attention by alignment.} 
According to Tables \ref{tab:1} and  \ref{tab:2}, the gains are in 2--5\% range compared to the baseline C3D SoSN.
% 
Figure \ref{fig:ssta_loss}a shows the training loss \wrt~epoch (HMDB51) ({\em temp. jigsaw}). Figure \ref{fig:ssta_loss}b shows the validation accuracy (HMDB51) \wrt~$\gamma$ for SS ({\em rot.}) As can be seen, Self-supervision combined with Attention by alignment (any curve for $\gamma\!>\!0$) scores higher than Self-supervision with Attention only ($\gamma\!=\!0$).




==> 3831 2/5-conclusion.tex <==
\section{Conclusions}
We have proposed a new few-shot Action Recognition Network (ARN) which comprises an encoder, comparator and an attention mechanism to model short- and long-range temporal patterns. We have investigated the role of self-supervision via spatial and temporal augmentations/auxiliary tasks. Moreover, we have proposed a novel mechanism dubbed {\em attention by alignment} which tackles the so-called distribution shift of temporal positions of discriminative long-range blocks. By combining losses of self-supervision and attention by alignment, we see gains of up to 6\% accuracy. We make our dataset splits publicly available to facilitate fair comparisons of few-shot action recognition pipelines.


==> 3831 2/definitions.tex <==
% variables
%\vec{\mathcal{M}}
\renewcommand\vec[1]{\ensuremath\boldsymbol{#1}}
\renewcommand\cdots{...}
\newcommand{\tB}{\vec{\mathcal{B}}}
\newcommand{\tD}{\vec{\mathcal{D}}}
\newcommand{\tY}{\vec{\mathcal{Y}}}
\newcommand{\tF}{\vec{\mathcal{F}}}
\newcommand{\tT}{\vec{\mathcal{T}}}
%\newcommand{\tS}{\vec{\mathcal{S}}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mZ}{\mathbf{Z}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\tX}{\vec{\mathcal{X}}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\mbrp}[1]{\mathbb{R}_{+}^{#1}}
\newcommand{\mbr}[1]{\mathbb{R}^{#1}}
\newcommand{\mbn}[1]{\mathbb{N}^{#1}}
\newcommand{\mbnz}[1]{\mathbb{N}_{0^+}^{#1}}
\newcommand{\mbnp}[1]{\mathbb{N}_{+}^{#1}}
\newcommand{\stackThree}{{;}_{3}}
\newcommand{\vbeta}{\vec{\beta}}
%\newcommand{\rank}[1]{\text{Rank}({#1})}

%\newcommand{\tXS}{\vec{\mathcal{X}}^{*}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\tV}{\vec{\mathcal{V}}}
\newcommand{\tE}{\vec{\mathcal{E}}}
\newcommand{\tEH}{\vec{\mathcal{\hat{E}}}}
\newcommand{\tVH}{\vec{\mathcal{\bar{V}}}}
\newcommand{\tVT}{\vec{\mathcal{\hat{V}}}}
\newcommand{\idx}[1]{\mathcal{I}_{#1}}
\newcommand{\semipd}[1]{\mathcal{S}_{+}^{#1}}
\newcommand{\spd}[1]{\mathcal{S}_{++}^{#1}}

\newcommand{\tR}{\vec{\mathcal{R}}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vup}{\mathbf{u^{'}}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vzeta}{\boldsymbol{\zeta}}
\newcommand{\vc}{\mathbf{c}}

\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vpsi}{\boldsymbol{\psi}}
\newcommand{\tPsi}{\vec{\mathcal{V}}}
\newcommand{\bigoh}{\mathcal{O}}
\newcommand{\mPsi}{\vec{\Psi}}
\newcommand{\vj}{\vec{j}}

% operators
\newcommand{\enorm}[1]{\left\|{#1}\right\|_2}
\newcommand{\fnorm}[1]{\left\|{#1}\right\|_F}
\newcommand{\lnorm}[1]{\left\|{#1}\right\|_1}
\newcommand{\riem}{\mathbf{d}_{\mathcal{R}}}
\newcommand{\spdp}[1]{\mathbb{S}_{++}^{#1}}
\newcommand{\simplex}[1]{\Delta^{#1}}
\newcommand{\set}[1]{\left\{#1\right\}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\supp}{Supp}
\DeclareMathOperator*{\unique}{Unique}
\DeclareMathOperator*{\TRank}{TRank}
\DeclareMathOperator*{\rank}{Rank}
\DeclareMathOperator*{\spann}{Span}
\DeclareMathOperator*{\sym}{Sym}

\newcommand{\flatt}[1]{\text{Flatten}\!\left({#1}\right)}
\newcommand{\unflatt}[1]{\text{Flatten}^{-1}\!\left({#1}\right)}
\newcommand{\myspan}[1]{\spann\left(#1\right)}

\DeclareMathOperator*{\trace}{Tr}
%\DeclareMathOperator*{\rank}{Rank}
\DeclareMathOperator*{\kronstack}{\uparrow\!\otimes}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\sgn}{Sgn}
\DeclareMathOperator*{\hosvd}{HOSVD}
\DeclareMathOperator*{\logm}{Log}
\DeclareMathOperator*{\detm}{Det}
\DeclareMathOperator*{\fg}{g}
\newcommand{\expl}[1]{\text{e}^{#1}}
\DeclareMathOperator*{\res}{Res}
\DeclareMathOperator*{\asinh}{Asinh}
%\newcommand{\exp}[1]{e^{#1}}




\newcommand{\mI}{\mathbf{I}}
\newcommand{\normvec}[1]{\frac{#1}{\|{#1}\|_2}}
\newcommand{\suptensor}[1]{\mathfrak{S}^{#1}}
\newcommand{\suptensorr}[2]{\mathfrak{S}^{#1}_{\times^{#2}}}
\newcommand{\region}{\mathcal{R}}

%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{remark}{Remark}

\newcommand{\todo}[1]{{\bf \textcolor{red}{[TODO: #1]}}}


\newcommand{\mLa}{\bm{\lambda}^{*}}
\newcommand{\mLambda}{\bm{\lambda}}
\newcommand{\mU}{\bm{U}}
\newcommand{\mV}{\bm{V}}
\newcommand{\timetplone}{{(t+1)}}
\newcommand{\timet}{{(t)}}

\newcommand{\mBOvl}{{\mB^{*}}}

\newcommand{\piA}{{\Pi_A}}
\newcommand{\piB}{{\Pi_B}}

\newcommand{\sigmav}{{^v\!\!\,{\sigma}}}
%\newcommand{\thickhat}[1]{\mathbf{\ddot{\text{$#1$}}}}
\newcommand{\sigmas}{{^s\!\!\,{\sigma}}}

\newcommand{\fvx}{{\boldsymbol{f}(\vx)}}
\newcommand{\fvy}{{\boldsymbol{f}(\vy)}}

\newcommand{\vsss}{\boldsymbol{s}}
\newcommand{\vw}{\boldsymbol{w}}

\newcommand{\vphibar}{\boldsymbol{\bar{\phi}}}
\newcommand{\vsigma}{\boldsymbol{\sigma}}

\def\eg{\emph{e.g.}}

\newcommand{\myg}[1]{\boldsymbol{G}\left(#1\right)}
\newcommand{\mygtwo}[1]{\boldsymbol{G}\Big(#1\Big)}
%\newcommand{\mygthree}[1]{\boldsymbol{G}\left(#1\right)}
\newcommand{\mygthree}[1]{\boldsymbol{\mathcal{G}}\!\left(\!#1\!\right)}
\newcommand{\mygfour}[1]{\boldsymbol{\mathcal{G}}\!\Bigg(\!#1\!\Bigg)}
\newcommand{\tG}{\boldsymbol{\mathcal{G}}}
\newcommand{\tP}{\boldsymbol{\mathcal{P}}}

\newcommand{\vPhi}{\boldsymbol{\Phi}}
\newcommand{\invbeta}{{(1\!-\!\beta)}}
\newcommand{\invsqrtbeta}{\sqrt{1\!-\!\beta}}
\newcommand{\sqrtbeta}{\sqrt{\beta}}


\newcommand{\mIdent}{\boldsymbol{\mathds{I}}}
\newcommand{\sIdent}{\mathds{I}}
\newcommand{\vOnes}{\mathbb{1}}

\newcommand{\mJ}{\mathbf{J}}
\newcommand{\sXkl}{{X_{kl}}}

\newcommand{\mK}{\mathbf{K}}
\newcommand{\mKb}{\bar{\mK}}
\newcommand{\mKbb}{\bar{\mKb}}
\newcommand{\Kb}{\bar{K}}
\newcommand{\Kbb}{\bar{\Kb}}
\newcommand{\mC}{\mathbf{C}}

\newcommand{\mKro}{{\mK^{q}}}
\newcommand{\mKbro}{{\mKb{\,\!}^{q}}}
\newcommand{\mKbbro}{{\mKbb^{q}}}
\newcommand{\Kbro}{{\Kb^{q}}}
\newcommand{\Kbbro}{{\Kbb^{q}}}



\newcommand{\fvxt}{{\boldsymbol{f}^{(t)}(\vx)}}
\newcommand{\Fvxt}{{\boldsymbol{F}^{(t)}(\vx)}}
\newcommand{\fvxtplusone}{{\boldsymbol{f}^{(t+1)}(\vx)}}
\newcommand{\Fvxtplusone}{{\boldsymbol{F}^{(t+1)}(\vx)}}
\newcommand{\vxzero}{\mathbf{x}_0}
\newcommand{\fvxzerotplusone}{{\boldsymbol{f}^{(t+1)}(\vxzero)}}
\newcommand{\Fvxzerotplusone}{{\boldsymbol{F}^{(t+1)}(\vxzero)}}
\newcommand{\fvxzerotplusonei}{{\boldsymbol{f}_i^{(t+1)}(\vxzero)}}

\newcommand{\tFvxt}{{{\vec{\mathcal{F}}}^{(t)}(\vx)}}
\newcommand{\tFvxtplusone}{{{\vec{\mathcal{F}}}^{(t+1)}(\vx)}}
\newcommand{\tFvxzerotplusone}{{{\vec{\mathcal{F}}}^{(t+1)}(\vxzero)}}




\newcommand{\swbar}{\bar{w}}
\newcommand{\vwbar}{\bar{\boldsymbol{w}}}

\newcommand{\vvartheta}{\boldsymbol{\vartheta}}
\newcommand{\tprim}[1]{{\uparrow T_{#1}}}


\newcommand{\vS}{\boldsymbol{S}}

\newcommand{\barM}{{\bar{M}}}
\newcommand{\barmM}{{\bar{\vec{M}}}}

\newcommand{\sN}{\vec{N}}
\newcommand{\tN}{\vec{\mathcal{N}}}
%\newcommand{\tP}{\vec{\mathcal{P}}}
\newcommand{\tS}{\vec{\mathcal{S}}}
\newcommand{\tSnb}{\mathcal{S}}
\newcommand{\mS}{\vec{S}}
\newcommand{\tNnb}{\mathcal{N}}

\newcommand{\cov}{\boldsymbol{\Sigma}}
\newcommand{\covb}{\boldsymbol{\Sigma}^{(\!\diamond\!)}}
\newcommand{\covw}{\boldsymbol{\Sigma}^{(\!*\!)}}
\newcommand{\vphix}[1]{{\boldsymbol{\phi}\left({#1}\right)}}
\newcommand{\covbb}[1]{{\boldsymbol{\Sigma}^{(\diamond,{#1})}}}
\newcommand{\covww}[1]{{\boldsymbol{\Sigma}_c^{(*,{#1})}}}

\newcommand{\muw}{\boldsymbol{\mu}^{(*)}}
\newcommand{\mub}{\boldsymbol{\mu}^{(\diamond)}}

\newcommand{\mubb}[1]{{\boldsymbol{\mu}^{(\diamond,{#1})}}}
\newcommand{\muww}[1]{{\boldsymbol{\mu}_c^{(*,{#1})}}}
\newcommand{\muwww}[2]{{\boldsymbol{\mu}_{#1}^{(*,{#2})}}}

\newcommand{\mPhi}{\boldsymbol{\Phi}}
\newcommand{\parsmP}{\!\left(\mPhi\right)}
\newcommand{\parsmPc}{\!\left(\mPhi_c\right)}
\newcommand{\parsmPA}{\!\left(\mPhi^A\right)}
\newcommand{\parsmPB}{\!\left(\mPhi^B\right)}
\newcommand{\parsmPAB}{\!\left(\mPhi^A\!,\mPhi^B\right)}
\newcommand{\parsmPcA}{\!\left(\mPhi_c^A\right)}
\newcommand{\parsmPcB}{\!\left(\mPhi_c^B\right)}
\newcommand{\parsmPxY}[2]{{\!\left(\mPhi_{#1}^{#2}\right)}}

\newcommand{\mMu}{\boldsymbol{M}}
\newcommand{\mM}{\boldsymbol{M}}
\newcommand{\parsmMu}{\!\left(\mMu\right)}
\newcommand{\mW}{\boldsymbol{W}}
\newcommand{\mD}{\boldsymbol{D}}
\newcommand{\mT}{\boldsymbol{T}}

\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\bvmu}{\boldsymbol{\overline{\mu}}}
\newcommand{\mP}{\boldsymbol{\Theta}}
\newcommand{\vmubar}{\boldsymbol{\bar{\mu}}}
\newcommand{\vvarphi}{\boldsymbol{\varphi}}


\newcommand{\stkout}[1]{{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}}

\newcommand{\mL}{\mathbf{L}}

\DeclareMathOperator*{\arcsinh}{arcsinh}
